OpenOOD v1.5: Enhanced Benchmark for Out-of-Distribution Detection

Out-of-Distribution (OOD) detection is critical for the reliable operation of open-world intelligent systems. Despite the emergence of an increasing number of OOD detection methods, the evaluation inconsistencies present challenges for tracking the progress in this field. OpenOOD v1 initiated the unification of the OOD detection evaluation but faced limitations in scalability and scope. In response, this paper presents OpenOOD v1.5, a significant improvement from its predecessor that ensures accurate and standardized evaluation of OOD detection methodologies at large scale. Notably, OpenOOD v1.5 extends its evaluation capabilities to large-scale data sets (ImageNet) and foundation models (e.g., CLIP and DINOv2), and expands its scope to investigate full-spectrum OOD detection which considers semantic and covariate distribution shifts at the same time. This work also contributes in-depth analysis and insights derived from comprehensive experimental results, thereby enriching the knowledge pool of OOD detection methodologies. With these enhancements, OpenOOD v1.5 aims to drive advancements and offer a more robust and comprehensive evaluation benchmark for OOD detection research.

==> tables/main_results_new.tex <==
\begin{table*}[th]
%\vspace{-1mm}
\centering
{\renewcommand\baselinestretch{1.3}\selectfont\resizebox{0.99\textwidth}{!}{
    \begin{tabular}{l|>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{1.8cm}|>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{1.8cm}|>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{1.8cm}|>{\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.6cm}} 
    \toprule
     & \multicolumn{3}{c|}{\textbf{CIFAR-10} {\color{gray} (ResNet-18)}} & \multicolumn{3}{c|}{\textbf{CIFAR-100} {\color{gray} (ResNet-18)}} & \multicolumn{3}{c|}{\textbf{ImageNet-200} {\color{gray} (ResNet-18)}} & \multicolumn{3}{c}{\textbf{ImageNet-1K} {\color{gray} (ResNet-50)}} \\
    
     & {\footnotesize Near-OOD} & {\footnotesize Far-OOD} & {\footnotesize ID Acc.} & {\footnotesize Near-OOD} & {\footnotesize Far-OOD} & {\footnotesize ID Acc.} & {\footnotesize Near-OOD} & {\footnotesize Far-OOD} & {\footnotesize ID Acc.} & {\footnotesize Near-OOD} & {\footnotesize Far-OOD} & {\footnotesize ID Acc.} \\
    \midrule

\multicolumn{7}{l}{\textbf{- Post-hoc Inference Methods}} \vspace{.1cm} \\

\rowcolor{NO_TRAIN} OpenMax 
{\footnotesize\cite{openmax16cvpr}} %(CVPR'16) 
& 87.62\textsubscript{(\textpm 0.29)} & 89.62\textsubscript{(\textpm 0.19)} & 95.06\textsubscript{(\textpm 0.30)} & 76.41\textsubscript{(\textpm 0.25)} & 79.48\textsubscript{(\textpm 0.41)} & 77.25\textsubscript{(\textpm 0.10)} & 80.27\textsubscript{(\textpm 0.10)} & 90.20\textsubscript{(\textpm 0.17)} & 86.37\textsubscript{(\textpm 0.08)} & 74.77 & 89.26 & 76.18 \\

\rowcolor{NO_TRAIN} MSP 
{\footnotesize\cite{msp17iclr}} %(ICLR'17) 
& 88.03\textsubscript{(\textpm 0.25)} & 90.73\textsubscript{(\textpm 0.43)} & 95.06\textsubscript{(\textpm 0.30)} & 80.27\textsubscript{(\textpm 0.11)} & 77.76\textsubscript{(\textpm 0.44)} & 77.25\textsubscript{(\textpm 0.10)} & 83.34\textsubscript{(\textpm 0.06)} & 90.13\textsubscript{(\textpm 0.09)} & 86.37\textsubscript{(\textpm 0.08)} & 76.02 & 85.23 & 76.18 \\

\rowcolor{NO_TRAIN} TempScale 
{\footnotesize\cite{guo2017calibration}} %(ICML'17) 
& 88.09\textsubscript{(\textpm 0.31)} & 90.97\textsubscript{(\textpm 0.52)} & 95.06\textsubscript{(\textpm 0.30)} & 80.90\textsubscript{(\textpm 0.07)} & 78.74\textsubscript{(\textpm 0.51)} & 77.25\textsubscript{(\textpm 0.10)} & \textbf{83.69}\textsubscript{(\textpm 0.04)} & 90.82\textsubscript{(\textpm 0.09)} & 86.37\textsubscript{(\textpm 0.08)} & 77.14 & 87.56 & 76.18 \\

\rowcolor{NO_TRAIN} ODIN 
{\footnotesize\cite{odin18iclr}} %(ICLR'18) 
& 82.87\textsubscript{(\textpm 1.85)} & 87.96\textsubscript{(\textpm 0.61)} & 95.06\textsubscript{(\textpm 0.30)} & 79.90\textsubscript{(\textpm 0.11)} & 79.28\textsubscript{(\textpm 0.21)} & 77.25\textsubscript{(\textpm 0.10)} & 80.27\textsubscript{(\textpm 0.08)} & 91.71\textsubscript{(\textpm 0.19)} & 86.37\textsubscript{(\textpm 0.08)} & 74.75 & 89.47 & 76.18 \\

\rowcolor{NO_TRAIN} MDS 
{\footnotesize\cite{mahananobis18nips}} %(NeurIPS'18) 
& 84.20\textsubscript{(\textpm 2.40)} & 89.72\textsubscript{(\textpm 1.36)} & 95.06\textsubscript{(\textpm 0.30)} & 58.69\textsubscript{(\textpm 0.09)} & 69.39\textsubscript{(\textpm 1.39)} & 77.25\textsubscript{(\textpm 0.10)} & 61.93\textsubscript{(\textpm 0.51)} & 74.72\textsubscript{(\textpm 0.26)} & 86.37\textsubscript{(\textpm 0.08)} & 55.44 & 74.25 & 76.18 \\

\rowcolor{NO_TRAIN} MDSEns {\footnotesize\cite{mahananobis18nips}} %(NeurIPS'18) 
& 60.43\textsubscript{(\textpm 0.26)} & 73.90\textsubscript{(\textpm 0.27)} & 95.06\textsubscript{(\textpm 0.30)} & 46.31\textsubscript{(\textpm 0.24)} & 66.00\textsubscript{(\textpm 0.69)} & 77.25\textsubscript{(\textpm 0.10)} & 54.32\textsubscript{(\textpm 0.24)} & 69.27\textsubscript{(\textpm 0.57)} & 86.37\textsubscript{(\textpm 0.08)} & 49.67 & 67.52 & 76.18 \\

\rowcolor{NO_TRAIN} RMDS 
{\footnotesize\cite{rmd21arxiv}} %(arXiv'21) 
& 89.80\textsubscript{(\textpm 0.28)} & 92.20\textsubscript{(\textpm 0.21)} & 95.06\textsubscript{(\textpm 0.30)} & 80.15\textsubscript{(\textpm 0.11)} & \textbf{82.92}\textsubscript{(\textpm 0.42)} & 77.25\textsubscript{(\textpm 0.10)} & 82.57\textsubscript{(\textpm 0.25)} & 88.06\textsubscript{(\textpm 0.34)} & 86.37\textsubscript{(\textpm 0.08)} & 76.99 & 86.38 & 76.18 \\

\rowcolor{NO_TRAIN} Gram 
{\footnotesize\cite{gram20icml}} %(ICML'20) 
& 58.66\textsubscript{(\textpm 4.83)} & 71.73\textsubscript{(\textpm 3.20)} & 95.06\textsubscript{(\textpm 0.30)} & 51.66\textsubscript{(\textpm 0.77)} & 73.36\textsubscript{(\textpm 1.08)} & 77.25\textsubscript{(\textpm 0.10)} & 67.67\textsubscript{(\textpm 1.07)} & 71.19\textsubscript{(\textpm 0.24)} & 86.37\textsubscript{(\textpm 0.08)} & 61.70 & 79.71 & 76.18 \\

\rowcolor{NO_TRAIN} EBO 
{\footnotesize\cite{energyood20nips}} %(NeurIPS'20) 
& 87.58\textsubscript{(\textpm 0.46)} & 91.21\textsubscript{(\textpm 0.92)} & 95.06\textsubscript{(\textpm 0.30)} & 80.91\textsubscript{(\textpm 0.08)} & 79.77\textsubscript{(\textpm 0.61)} & 77.25\textsubscript{(\textpm 0.10)} & 82.50\textsubscript{(\textpm 0.05)} & 90.86\textsubscript{(\textpm 0.21)} & 86.37\textsubscript{(\textpm 0.08)} & 75.89 & 89.47 & 76.18 \\

\rowcolor{NO_TRAIN} OpenGAN {\footnotesize\cite{kong2021opengan}} %(ICCV'21) 
& 53.71\textsubscript{(\textpm 7.68)} & 54.61\textsubscript{(\textpm 15.51)} & 95.06\textsubscript{(\textpm 0.30)} & 65.98\textsubscript{(\textpm 1.26)} & 67.88\textsubscript{(\textpm 7.16)} & 77.25\textsubscript{(\textpm 0.10)} & 59.79\textsubscript{(\textpm 3.39)} & 73.15\textsubscript{(\textpm 4.07)} & 86.37\textsubscript{(\textpm 0.08)} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} \\

\rowcolor{NO_TRAIN} GradNorm 
{\footnotesize \cite{gradnorm21nips}} %(NeurIPS'21) 
& 54.90\textsubscript{(\textpm 0.98)} & 57.55\textsubscript{(\textpm 3.22)} & 95.06\textsubscript{(\textpm 0.30)} & 70.13\textsubscript{(\textpm 0.47)} & 69.14\textsubscript{(\textpm 1.05)} & 77.25\textsubscript{(\textpm 0.10)} & 72.75\textsubscript{(\textpm 0.48)} & 84.26\textsubscript{(\textpm 0.87)} & 86.37\textsubscript{(\textpm 0.08)} & 72.96 & 90.25 & 76.18 \\

\rowcolor{NO_TRAIN} ReAct 
{\footnotesize\cite{react21nips}} %(NeurIPS'21) 
& 87.11\textsubscript{(\textpm 0.61)} & 90.42\textsubscript{(\textpm 1.41)} & 95.06\textsubscript{(\textpm 0.30)} & 80.77\textsubscript{(\textpm 0.05)} & 80.39\textsubscript{(\textpm 0.49)} & 77.25\textsubscript{(\textpm 0.10)} & 81.87\textsubscript{(\textpm 0.98)} & 92.31\textsubscript{(\textpm 0.56)} & 86.37\textsubscript{(\textpm 0.08)} & 77.38 & 93.67 & 76.18 \\

\rowcolor{NO_TRAIN} MLS 
{\footnotesize\cite{species22icml}} %(ICML'22) 
& 87.52\textsubscript{(\textpm 0.47)} & 91.10\textsubscript{(\textpm 0.89)} & 95.06\textsubscript{(\textpm 0.30)} & \textbf{81.05}\textsubscript{(\textpm 0.07)} & 79.67\textsubscript{(\textpm 0.57)} & 77.25\textsubscript{(\textpm 0.10)} & 82.90\textsubscript{(\textpm 0.04)} & 91.11\textsubscript{(\textpm 0.19)} & 86.37\textsubscript{(\textpm 0.08)} & 76.46 & 89.57 & 76.18 \\

\rowcolor{NO_TRAIN} KLM 
{\footnotesize\cite{species22icml}} %(ICML'22) 
& 79.19\textsubscript{(\textpm 0.80)} & 82.68\textsubscript{(\textpm 0.21)} & 95.06\textsubscript{(\textpm 0.30)} & 76.56\textsubscript{(\textpm 0.25)} & 76.24\textsubscript{(\textpm 0.52)} & 77.25\textsubscript{(\textpm 0.10)} & 80.76\textsubscript{(\textpm 0.08)} & 88.53\textsubscript{(\textpm 0.11)} & 86.37\textsubscript{(\textpm 0.08)} & 76.64 & 87.60 & 76.18 \\

\rowcolor{NO_TRAIN} VIM 
{\footnotesize\cite{haoqi2022vim}} %(CVPR'22) 
& 88.68\textsubscript{(\textpm 0.28)} & \textbf{93.48}\textsubscript{(\textpm 0.24)} & 95.06\textsubscript{(\textpm 0.30)} & 74.98\textsubscript{(\textpm 0.13)} & 81.70\textsubscript{(\textpm 0.62)} & 77.25\textsubscript{(\textpm 0.10)} & 78.68\textsubscript{(\textpm 0.24)} & 91.26\textsubscript{(\textpm 0.19)} & 86.37\textsubscript{(\textpm 0.08)} & 72.08 & 92.68 & 76.18 \\

\rowcolor{NO_TRAIN} KNN 
{\footnotesize\cite{sun2022knnood}} %(ICML'22) 
& \textbf{90.64}\textsubscript{(\textpm 0.20)} & 92.96\textsubscript{(\textpm 0.14)} & 95.06\textsubscript{(\textpm 0.30)} & 80.18\textsubscript{(\textpm 0.15)} & 82.40\textsubscript{(\textpm 0.17)} & 77.25\textsubscript{(\textpm 0.10)} & 81.57\textsubscript{(\textpm 0.17)} & 93.16\textsubscript{(\textpm 0.22)} & 86.37\textsubscript{(\textpm 0.08)} & 71.10 & 90.18 & 76.18 \\

\rowcolor{NO_TRAIN} DICE 
{\footnotesize\cite{sun2021dice}} %(ECCV'22) 
& 78.34\textsubscript{(\textpm 0.79)} & 84.23\textsubscript{(\textpm 1.89)} & 95.06\textsubscript{(\textpm 0.30)} & 79.38\textsubscript{(\textpm 0.23)} & 80.01\textsubscript{(\textpm 0.18)} & 77.25\textsubscript{(\textpm 0.10)} & 81.78\textsubscript{(\textpm 0.14)} & 90.80\textsubscript{(\textpm 0.31)} & 86.37\textsubscript{(\textpm 0.08)} & 73.07 & 90.95 & 76.18 \\

\rowcolor{NO_TRAIN} RankFeat 
{\footnotesize\cite{song2022rankfeat}} %(NeurIPS'22) 
& 79.46\textsubscript{(\textpm 2.52)} & 75.87\textsubscript{(\textpm 5.06)} & 95.06\textsubscript{(\textpm 0.30)} & 61.88\textsubscript{(\textpm 1.28)} & 67.10\textsubscript{(\textpm 1.42)} & 77.25\textsubscript{(\textpm 0.10)} & 56.92\textsubscript{(\textpm 1.59)} & 38.22\textsubscript{(\textpm 3.85)} & 86.37\textsubscript{(\textpm 0.08)} & 50.99 & 53.93 & 76.18 \\

\rowcolor{NO_TRAIN} ASH 
{\footnotesize\cite{djurisic2023extremely}} %(ICLR'23) 
& 75.27\textsubscript{(\textpm 1.04)} & 78.49\textsubscript{(\textpm 2.58)} & 95.06\textsubscript{(\textpm 0.30)} & 78.20\textsubscript{(\textpm 0.15)} & 80.58\textsubscript{(\textpm 0.66)} & 77.25\textsubscript{(\textpm 0.10)} & 82.38\textsubscript{(\textpm 0.19)} & \textbf{93.90}\textsubscript{(\textpm 0.27)} & 86.37\textsubscript{(\textpm 0.08)} & \textbf{78.17} & \textbf{95.74} & 76.18 \\

\rowcolor{NO_TRAIN} SHE \cite{she23iclr} %(ICLR'23) 
& 81.54\textsubscript{(\textpm 0.51)} & 85.32\textsubscript{(\textpm 1.43)} & 95.06\textsubscript{(\textpm 0.30)} & 78.95\textsubscript{(\textpm 0.18)} & 76.92\textsubscript{(\textpm 1.16)} & 77.25\textsubscript{(\textpm 0.10)} & 80.18\textsubscript{(\textpm 0.25)} & 89.81\textsubscript{(\textpm 0.61)} & 86.37\textsubscript{(\textpm 0.08)} & 73.78 & 90.92 & 76.18 \\


\multicolumn{7}{l}{\textbf{- Training Methods (w/o Outlier Data)}} \vspace{.1cm} \\

\rowcolor{NEED_TRAIN} ConfBranch 
{\footnotesize\cite{confbranch2018arxiv}} %(arXiv'18) 
& 89.84\textsubscript{(\textpm 0.24)} & 92.85\textsubscript{(\textpm 0.29)} & 94.88\textsubscript{(\textpm 0.05)} & 71.60\textsubscript{(\textpm 0.62)} & 68.90\textsubscript{(\textpm 1.83)} & 76.59\textsubscript{(\textpm 0.27)} & 79.10\textsubscript{(\textpm 0.24)} & 90.43\textsubscript{(\textpm 0.18)} & 85.92\textsubscript{(\textpm 0.07)} & 70.66 & 83.94 & 75.63 \\

\rowcolor{NEED_TRAIN} RotPred 
{\footnotesize\cite{rotpred}} %(NeurIPS'19) 
& \textbf{92.68}\textsubscript{(\textpm 0.27)} & 96.62\textsubscript{(\textpm 0.18)} & \textbf{95.35}\textsubscript{(\textpm 0.52)} & 76.43\textsubscript{(\textpm 0.16)} & \textbf{88.40}\textsubscript{(\textpm 0.13)} & 76.03\textsubscript{(\textpm 0.38)} & 81.59\textsubscript{(\textpm 0.20)} & 92.56\textsubscript{(\textpm 0.09)} & \textbf{86.37}\textsubscript{(\textpm 0.16)} & \textbf{76.52} & 90.00 & \textbf{76.55} \\

\rowcolor{NEED_TRAIN} G-ODIN 
{\footnotesize\cite{godin20cvpr}} %(CVPR'20) 
& 89.12\textsubscript{(\textpm 0.57)} & 95.51\textsubscript{(\textpm 0.31)} & 94.70\textsubscript{(\textpm 0.25)} & 77.15\textsubscript{(\textpm 0.28)} & 85.67\textsubscript{(\textpm 1.58)} & 74.46\textsubscript{(\textpm 0.04)} & 77.28\textsubscript{(\textpm 0.10)} & 92.33\textsubscript{(\textpm 0.11)} & 84.56\textsubscript{(\textpm 0.28)} & 70.77 & 85.51 & 74.85 \\

\rowcolor{NEED_TRAIN} CSI 
{\footnotesize\cite{csi20nips}} %(NeurIPS'20) 
& 89.51\textsubscript{(\textpm 0.19)} & 92.00\textsubscript{(\textpm 0.30)} & 91.16\textsubscript{(\textpm 0.14)} & 71.45\textsubscript{(\textpm 0.27)} & 66.31\textsubscript{(\textpm 1.21)} & 61.60\textsubscript{(\textpm 0.46)} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} \\

\rowcolor{NEED_TRAIN} ARPL 
{\footnotesize\cite{arpl2021pami}} %(TPAMI'21) 
& 87.44\textsubscript{(\textpm 0.15)} & 89.31\textsubscript{(\textpm 0.32)} & 93.66\textsubscript{(\textpm 0.11)} & 74.94\textsubscript{(\textpm 0.93)} & 73.69\textsubscript{(\textpm 1.80)} & 70.70\textsubscript{(\textpm 1.08)} & 82.02\textsubscript{(\textpm 0.10)} & 89.23\textsubscript{(\textpm 0.11)} & 83.95\textsubscript{(\textpm 0.32)} & 76.30 & 85.50 & 75.87 \\

\rowcolor{NEED_TRAIN} MOS {\footnotesize \cite{mos21cvpr}} %(CVPR'21) 
& 71.45\textsubscript{(\textpm 3.09)} & 76.41\textsubscript{(\textpm 5.93)} & 94.83\textsubscript{(\textpm 0.37)} & 80.40\textsubscript{(\textpm 0.18)} & 80.17\textsubscript{(\textpm 1.21)} & 76.98\textsubscript{(\textpm 0.20)} & 69.84\textsubscript{(\textpm 0.46)} & 80.46\textsubscript{(\textpm 0.92)} & 85.60\textsubscript{(\textpm 0.20)} & 72.85 & 82.75 & 72.81 \\

\rowcolor{NEED_TRAIN} VOS 
{\footnotesize \cite{vos22iclr}} %(ICLR'22)
& 87.70\textsubscript{(\textpm 0.48)} & 90.83\textsubscript{(\textpm 0.92)} & 94.31\textsubscript{(\textpm 0.64)} & \textbf{80.93}\textsubscript{(\textpm 0.29)} & 81.32\textsubscript{(\textpm 0.09)} & 77.20\textsubscript{(\textpm 0.10)} & 82.51\textsubscript{(\textpm 0.11)} & 91.00\textsubscript{(\textpm 0.28)} & 86.23\textsubscript{(\textpm 0.19)} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} \\

\rowcolor{NEED_TRAIN} LogitNorm 
{\footnotesize \cite{wei2022mitigating}} %(ICML'22)
& 92.33\textsubscript{(\textpm 0.08)} & \textbf{96.74}\textsubscript{(\textpm 0.06)} & 94.30\textsubscript{(\textpm 0.25)} & 78.47\textsubscript{(\textpm 0.31)} & 81.53\textsubscript{(\textpm 1.26)} & 76.34\textsubscript{(\textpm 0.17)} & \textbf{82.66}\textsubscript{(\textpm 0.15)} & 93.04\textsubscript{(\textpm 0.21)} & 86.04\textsubscript{(\textpm 0.15)} & 74.62 & 91.54 & 76.45 \\

\rowcolor{NEED_TRAIN} CIDER 
{\footnotesize \cite{cider2023iclr}} %(ICLR'23) 
& 90.71\textsubscript{(\textpm 0.16)} & 94.71\textsubscript{(\textpm 0.36)} & \textcolor{gray}{N/A} & 73.10\textsubscript{(\textpm 0.39)} & 80.49\textsubscript{(\textpm 0.68)} & \textcolor{gray}{N/A} & 80.58\textsubscript{(\textpm 1.75)} & 90.66\textsubscript{(\textpm 1.68)} & \textcolor{gray}{N/A} & 68.97 & \textbf{92.18} & \textcolor{gray}{N/A} \\

\rowcolor{NEED_TRAIN} NPOS 
{\footnotesize \cite{npos2023iclr}} %(ICLR'23) 
& 89.78\textsubscript{(\textpm 0.33)} & 94.07\textsubscript{(\textpm 0.49)} & \textcolor{gray}{N/A} & 78.35\textsubscript{(\textpm 0.37)} & 82.29\textsubscript{(\textpm 1.55)} & \textcolor{gray}{N/A} & 79.40\textsubscript{(\textpm 0.39)} & \textbf{94.49}\textsubscript{(\textpm 0.07)} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} \\


\multicolumn{7}{l}{\textbf{- Training Methods (w/ Outlier Data)}} \vspace{.1cm} \\

\rowcolor{EXTRA_DATA} OE 
{\footnotesize \cite{oe18nips}} %%(NeurIPS'18) 
& \textbf{94.82}\textsubscript{(\textpm 0.21)} & \textbf{96.00}\textsubscript{(\textpm 0.13)} & 94.63\textsubscript{(\textpm 0.26)} & \textbf{88.30}\textsubscript{(\textpm 0.10)} & \textbf{81.41}\textsubscript{(\textpm 1.49)} & \textbf{76.84}\textsubscript{(\textpm 0.42)} & \textbf{84.84}\textsubscript{(\textpm 0.16)} & \textbf{89.02}\textsubscript{(\textpm 0.18)} & 85.82\textsubscript{(\textpm 0.21)} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} \\

\rowcolor{EXTRA_DATA} MCD 
{\footnotesize \cite{mcd19iccv}} %(ICCV'19) 
& 91.03\textsubscript{(\textpm 0.12)} & 91.00\textsubscript{(\textpm 1.10)} & 94.95\textsubscript{(\textpm 0.04)} & 77.07\textsubscript{(\textpm 0.32)} & 74.72\textsubscript{(\textpm 0.78)} & 75.83\textsubscript{(\textpm 0.04)} & 83.62\textsubscript{(\textpm 0.09)} & 88.94\textsubscript{(\textpm 0.10)} & \textbf{86.12}\textsubscript{(\textpm 0.17)} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} \\

\rowcolor{EXTRA_DATA} UDG 
{\footnotesize \cite{yang2021scood}} %(ICCV'21) 
& 89.91\textsubscript{(\textpm 0.25)} & 94.06\textsubscript{(\textpm 0.90)} & 92.36\textsubscript{(\textpm 0.84)} & 78.02\textsubscript{(\textpm 0.10)} & 79.59\textsubscript{(\textpm 1.77)} & 71.54\textsubscript{(\textpm 0.64)} & 74.30\textsubscript{(\textpm 1.63)} & 82.09\textsubscript{(\textpm 2.78)} & 68.11\textsubscript{(\textpm 1.24)} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} \\

\rowcolor{EXTRA_DATA} MixOE 
{\footnotesize \cite{mixoe23wacv}} %(WACV'23) 
& 88.73\textsubscript{(\textpm 0.82)} & 91.93\textsubscript{(\textpm 0.69)} & 94.55\textsubscript{(\textpm 0.32)} & 80.95\textsubscript{(\textpm 0.20)} & 76.40\textsubscript{(\textpm 1.44)} & 75.13\textsubscript{(\textpm 0.06)} & 82.62\textsubscript{(\textpm 0.03)} & 88.27\textsubscript{(\textpm 0.41)} & 85.71\textsubscript{(\textpm 0.07)} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} & \textcolor{gray}{N/A} \\

\bottomrule
    \end{tabular}}\par}
\caption{Main results from OpenOOD v1.5 on standard OOD detection. In this table we use AUROC as the metric for OOD detection. Whenever applicable, we report the average number and the corresponding standard deviation obtained from 3 training runs. The best result within each group is bolded.
Results for data augmentation methods are listed in \cref{tab:inet_data_aug}. 
Full result table including other metrics and per-dataset statistics can be found in an online sheet (see \cref{fn_fullresults}).}
\label{tab:main_results}
\end{table*}


